QActor: On-line Active Learning for Noisy Labeled Stream Data

Noisy labeled data is more a norm than a rarity for self-generated content that is continuously published on the web and social media. Due to privacy concerns and governmental regulations, such a data stream can only be stored and used for learning purposes in a limited duration. To overcome the noise in this on-line scenario we propose QActor which novel combines: the selection of supposedly clean samples via quality models and actively querying an oracle for the most informative true labels. While the former can suffer from low data volumes of on-line scenarios, the latter is constrained by the availability and costs of human experts. QActor swiftly combines the merits of quality models for data filtering and oracle queries for cleaning the most informative data. The objective of QActor is to leverage the stringent oracle budget to robustly maximize the learning accuracy. QActor explores various strategies combining different query allocations and uncertainty measures. A central feature of QActor is to dynamically adjust the query limit according to the learning loss for each data batch. We extensively evaluate different image datasets fed into the classifier that can be standard machine learning (ML) models or deep neural networks (DNN) with noise label ratios ranging between 30% and 80%. Our results show that QActor can nearly match the optimal accuracy achieved using only clean data at the cost of at most an additional 6% of ground truth data from the oracle.

==> IJCAI-Evaluation.tex <==
\section{Experimental Setup}
Here we describe the datasets, the model parameters and the baselines used for comparison.

\subsection{Datasets}
We consider image datasets using the pixel values as inputs.
%and a deep learning approach which integrates feature selection into the training process.
In particular we use the well-known CIFAR-10 and CIFAR-100 datasets. These datasets try to classify colored $32\times32$-pixel images into ten and hundred classes, respectively.
CIFAR-100 is more complex due to both the higher number of classes.
Table~\ref{tab:datasets} summarises the characteristics of both datasets.

\subsection{Label Noise}
We inject label noise into the training set by corrupting the label of randomly sampled data instances. We term the sampling probability as noise rate. Corrupted samples are subject to symmetric noise, e.g., the true label is exchanged with a random different label with uniform probability. We consider noise rates of $30\%$ and $60\%$. Test data is not subject to label noise.


\subsection{Baselines}
\label{ssec:baselines}

To better show the overall effectiveness of our proposed \alg method we compare it two sets of baselines. First we compare against different active query selection baselines:

\begin{itemize}
    \item[] \textbf{{No-Sel}}: uses all samples that arrive in the batch to train the classifier without filtering.

    \item[] \textbf{{Q-only}}: in this case the quality model filters the suspicious samples but there is no active learner to relabel the informative noisy instances. Therefore the classifier will train only on the clean data instances identified by the quality model.

    \item[] \textbf{{AL-only}}: here there is no quality model to separate the clean from suspicious data instances. The classifier is trained without the quality model filtering the data, however, informative instances identified by the active learner are relabeled by the oracle.

    \item[] \textbf{{Opt-Sel}}: which assumes a perfect quality model able to identify all the true clean and noisy samples and uses all the clean samples for training the classifier without active learning.
\end{itemize}

Second we put \alg in the context of other noise-resistant techniques drawn from the related work on learning with noise and adapted to the online scenario:

\begin{itemize}
    \item[] \textbf{D2L}~\cite{wang2018iterative}: estimates the dimensionality of subspaces during training to adapt the loss function.
    \item[] \textbf{Forward}~\cite{patrini2017making}: corrects the loss function based on the noise transition matrix.
    \item[] \textbf{Bootstrap}~\cite{iclrw2015reed}: using convex combination of the given and predicted labels for training.
    \item[] \textbf{Co-teaching}~\cite{han2018co}: exchanges mini-batches between two networks trained in parallel.
\end{itemize}

\begin{table}[t]
\centering
\caption{Summary of main properties of evaluated datasets.}
\label{tab:datasets}
\begin{tabular}{l|cc}
\hline
Dataset          & {\bf CIFAR-10} & {\bf CIFAR-100}\\ \hline \hline
\# classes  $C$  & 10       & 100    \\
\# features $K$  & 32x32x3  & 32x32x3  \\ \hline
\# train images  & 50000    & 50000\\
\multicolumn{1}{r|}{per class}  & 5000    & 500\\ \hline
\# test images   & 10000    & 10000 \\ 
\multicolumn{1}{r|}{per class}   & 1000    & 100 \\ \hline
\end{tabular}
\end{table}

\input{bigtable_cifar.tex}

\subsection{Model Parameters}
As \alg classifier for CIFAR-10 and CIFAR-100 we use the two Convolutional Neural Network (CNN) architectures defined in~\cite{wang2018iterative} with ReLU activation functions, softmax activation as image classifier and cross-entropy as loss function. We train the models by using stochastic gradient descent with momentum $0.9$, learning rate $0.01$, and weight decay $10^{-4}$. \alg and all baselines are implemented using Keras v2.2.4 and Tensorflow v1.12, except co-teaching which uses PyTorch v1.1.0.

With CIFAR-10 \alg is trained initially with clean 10000 instances and 60 epochs. The remaining 40000 instances come in batches of size 1000 with $30\%$ ($60\%$) noise. Under static policy, in each batch we query $50$ ($100$) samples, i.e. $5\%$ ($10\%$) of the batch size, actively from the oracle and retrain the model for $20$ epochs. Similarly, the dynamic policy uses $B$ equal to only $5\%$ of the total noisy data. At the end of each batch, we test the model with the test set of 10000 instances. Rollback uses $a$ = 20\%. For CIFAR-100 we increase the arriving data batch size to 10000 and 60 epochs per batch to cope with the higher complexity.
For fair comparison, baselines are also trained under the same data arrival pattern and the same CNN structure. All baselines use the same parameters as from their papers except for D2L. Here we reduce the dimensionality estimation interval to 40 and 10 for the initial and subsequent batches, respectively. This keeps roughly the original ratio against the overall training period.
%With this number of epochs, the training accuracy is near $100\%$.
%\rb{We repeat each experiment for 3 times}
For each experiment we report the average accuracy covering the last received 10000 samples.

==> IJCAI-Introduction.tex <==
\section{Introduction}

We are in the era of big data, which are continuously generated on different web platforms, e.g., social media, and disseminated via search engines often in a casual and unstructured way. Consequently, such a big data experience suffers from diversified quality issues, e.g., images tagged with incorrect labels, so called noisy labels. Today's easy access to this large amount of data further exasperates the presence of extremely noisy data. According to~\cite{baddata}, noisy data costs the US industry more than \$3 trillion per year to cleanse or to mitigate the impact of derived incorrect analyses. While the learning models conveniently leverage such a free source of data, its quality greatly undermines the learning efficiencies and their associate utilities~\cite{jiang2017mentornet}. For example~\cite{Zhang2017memorization}, using an image classifier trained from data with highly noisy labels can significantly degrade classification accuracy and hinder its applicability on different domains.

Another challenge brought by big data is the stream of data generation and continuous data curation. On the one hand, this invalidates the assumptions of off-line learning scenarios and drastically increases the storage overhead. On the other hand, due to the privacy concern and government regulation, e.g., European GDPR, data shall be closely managed, imposing a limit on using curated data from the public domains.
% As such, today's machine learning models, e.g., classifying images, in reality often encounter such data that arrives in a stream of high velocity and can only be kept for a limited time.
As such, today's machine learning models, in reality often encounter stream data of high velocity allowing for only brief usage times, and affected by high amounts of wrong annotations. %due to automatic labeling.
% For instance, emerging tweet-based analyses~\cite{BarbosaF10ICCL}
% are subject to the risk of using streams of tweets that have high labelling noise.
% As mentioned in~\cite{EbrahimiDL16EMNLP}, ``his \#MakeAmericaGreatAgain \#Tag is a bumme'' is
% against Donald Trump, but was incorrectly labeled as favorable. The same issue happens with
For instance, emerging trend analyses~\cite{FerraraIT14Ht} are subject to the risk of using streams of data from Instagram and Twitter that have high labeling noise~\cite{BarbosaF10ICCL}.
As mentioned in~\cite{EbrahimiDL16EMNLP}, ``his \#MakeAmericaGreatAgain \#Tag is a bummer'' is
against Donald Trump, but was incorrectly labeled as favorable.
Furthermore, adversarial manipulations by attackers~\cite{goodfellow2014explaining} are another source of label noise in stream data. It is no mean feat to derive learning models which can cater to such a multi-faced challenge.
%, i.e., noisy stream data.
Our proposed method is highly relevant to these challenging situations of noisy stream data.

Noisy label issue has been a long standing challenge~\cite{patrini2017making}, from standard machine learning (ML) models to the recent deep neural networks (DNN), whose large learning capacities can have detrimental memorization effects on dirty labels~\cite{Zhang2017memorization}. The central theme here is to filter out the suspicious data which might have corrupted labels via quality estimates. Although such approaches show promising results in combating noisy labels, the applicability to noisy stream data is unfortunately limited, due to their assumption of off-line and complete data availability. The other drawback of filtering approaches is the risk of dropping informative data points which can be influential for the underlying learning models.
%For instance, images with corrupted labels can be exactly on the class boundaries.
It might be worthwhile to actively cleanse such data due to its high potential in improving the learning tasks, even at a certain expense.

Active learning techniques~\cite{settles2009active} are designed to query extra information from an oracle for the data whose (true) labels are not readily available. Such an oracle is assumed to know the ground truth, but at high costs, e.g. a human expert. Hence, only the informative/uncertain data is queried within a certain query budget. The majority of active learning approaches focus on the off-line scenario and constant budget, except~\cite{vzliobaite2013active} that explores active learning on one by one drifting streaming data.
%Motivated by its power of cleansing data, \cite{bouguelia2015stream} applies active learning techniques on support vector machines which encounter moderate  noise ratios, i.e., roughly 30\%.
The efficacy of active learning relies on identifying the most informative instances based on uncertainty measurements of learning tasks, e.g., class probability~\cite{schohn2000less}, entropy value~\cite{holub2008entropy} or posterior predictive densities~\cite{ijcai2019haussmann}. While the related work shows promising results of active learning on noisy labels, it is not clear how active query approach can be adopted when encountering noisy data streams that can be learnt only for a short period of time.

In this paper, we focus on a challenging multi-class learning problem whose data is streamed and its labels are extremely noisy, i.e., more than half of the given labels of streaming data are wrong. Due to privacy concerns and limited storage, data can only be stored for a limited amount of epochs, drastically shortening the data validity for training classifiers. In other words, only a small fraction of data is available for learning the model at any point in time, compared to the offline scenario. Our objective is to enhance the noise-resiliency of the underlying classifier by selectively learning from good data as well as noisy labels that are critical to train the classifier. In order to turn the noisy labels into a learning advantage, we resort to the oracle for recovering their label ground truth under a given query budget. Ultimately, we aim to optimize classification accuracy with a minimum number of oracle queries.%, in combating stream of noisy labels. 

To such an end, we design an on-line active learning framework, termed Quality-driven Active Learning (\alg), 
% which combines the merits of quality models and typical active learning algorithms.
which marries quality models with active learning.
Upon receiving new data instances, \alg first filters it via the quality model into ``clean'' and ``noisy'' categories. Second, \alg queries the oracle for the true labels of highly uncertain and informative noisy instances. % , determined by \todo{fill in the definition}.
Another unique feature of \alg is that the overall query budget is fixed but the number of queries per batch is 
dynamically adjusted based on the current training loss value. \alg uses more queries when the loss value increases to avoid incorrectly including noisy labels, and reduced otherwise. We extensively evaluate \alg on an extensive set of scenarios, i.e., noise ratios, %multi-class classifier models,
uncertain measures, and more importantly different data sets.
%\rb{
Our results show that in the presence of very large label noise, i.e., up to 60\% corrupted labels, \alg can achieve remarkable accuracy, i.e., almost match the optimal accuracy obtained excluding all noisy labels, at the cost of just a small fraction of oracle information, i.e., up to 5\% oracle queried labels. Moreover, compared to state of the art on noise resilient DNN, \alg achieves higher accuracy by 15\% and 10\% for CIFAR-10 and CIFAR-100, respectively.
%}

Our contributions are three fold. We design a novel and efficient learning framework, termed \alg,  whose core combines a quality model with on-line active learning. Secondly, we propose a dynamic learning strategy that can adapt to the dynamic nature of the online data and achieve better results as the static one. %\tr{
To the best of our knowledge, this is the first study on dynamic allocation of active learning budget in an online manner.%}. Thirdly, we extensively evaluate the proposed \alg on an extensive set of scenarios and datasets, strongly arguing for the combination of human and artificial intelligence.

==> IJCAI-Method.tex <==
\section{Quality-driven Active Learning \alg}
\subsection{Problem Statement}
We consider multi-class classification problems that map data inputs $x$ of $K$ features into labels $y$ of $C$ classes, $\mathbf{x} \in \mathbf{X}^{N \times K} $ into $y \in \bf{C}=\{1, \dots, \textit{C}\}$. A small set of initial data instances with clean labels used as initial seed is given, together with a testing set for evaluation. A clean data instance refers to a sample whose given label is properly annotated, without any alteration. A noisy data instance refers to samples whose label is corrupted, i.e. different from the true label.
Data instances are continuously collected over time. Specifically, we introduce $i$ and $t$ to denote a particularly data instance $i$ of data arriving at interval $t$ as $\mathbf{x}(t)_i$. For simplicity, we omit $t$ when referring $\mathbf{x}$. Algorithm 1 shows the overview of our proposed method. 

 \begin{figure}[tp]
    \centering
    \includegraphics[width=0.9\columnwidth]{Figures/alg_qactor.pdf}
    \caption{Overview of \alg: workflow of quality model, active learner, and classifier.}
    \label{fig:method}
\end{figure}

\subsection{Architecture of \alg}
Fig.~\ref{fig:method} depicts the architecture. The main components are the quality model $\mathfrak{Q}: \mathbf{x}\rightarrow y \in \mathbf{C}$, the label comparator which discerns noisy from clean labels, the active leaner which determines which and how many data instances to send to the oracle, and the classifier $\mathfrak{C}: \mathbf{\tilde{x}}\rightarrow y \in \mathbf{C}$. $\mathbf{\tilde{x}}$ is a subset of $\mathbf{x}$ defined below.

At each time $t$ the incoming data $x$ is first sent to the quality model from the previous time instance $\mathfrak{Q}(t-1)$  which predicts their labels. If the predicted labels are the same as the given ones, the label comparator marks them and their labels as clean, denoted as $\mathbf{x}^{cl}$; otherwise as noisy, $\mathbf{x}^{ny}$.
Noisy data instances are sent to the active learner to rank them and select $o(t)$ data instances $\mathbf{x}^{or}$ to send to oracle to query their true label. $o(t)$ is limited by the given available budget $B$, i.e., $\sum_t o(t) \le B$. Since $o(t)$ is typically much smaller than the number of noisy data instances, i.e. $o(t) \ll |\mathbf{x}^{ny}|$, instances are ranked and selected based on a uncertainty metric.
The clean and oracle relabeled instances are denoted by $\mathbf{\tilde{x}} = \mathbf{x}^{ny} \cup \mathbf{x}^{or}$ and used to re-train $\mathfrak{C}(t)$ and $\mathfrak{Q}(t)$. To avoid pitfalls in learning we monitor the accuracy on a small hold-out of the initial set. If performance drops by more than $a$ we roll back the model before processing the next data batch.

We use Deep Neural Networks (DNN) as classifier since they have shown extremely promising results in classifying complex image datasets~\cite{goodfellow2014explaining}. Due to the high training costs of deep neural networks, to reduce the computational burden, instead of having two different models for $\mathfrak{Q}$ and $\mathfrak{C}$, we leverage the time difference between data arrivals to use the previously trained $\mathfrak{C}$ as $\mathfrak{Q}$ for the following time period, i.e., $\mathfrak{Q}(t) = \mathfrak{C}(t-1)$. This optimization allows us to train only one model per time period.

\subsection{Uncertainty Measure}
\label{ssec:uncertainty}

We estimate the prediction uncertainty of DNN via the prediction probabilities $P$ at the output of the softmax layer. In general the higher the probability the more confident the prediction, but also how spread out the probability distribution is counts. Hence, we test three different uncertainty metrics: two drawn from the classic active-learning literature, plus one based on the training loss function of the DNN. Here, we use $P_{best}$ and $P_{second-best}$ to denote the probabilities of the most likely and second most likely class.

\begin{enumerate}
  \item \textbf{Least Confident (LC)} queries the instance where the model has the lowest classification confidence, i.e. $\min {P_{best}(\mathbf{x_i^{ny}})}$.
  \item \textbf{Best-versus-second-best (BvSB)}~\cite{joshi2009multi} considers instances where the difference between the two most likely classes is minimum meaning that these instances could have easily been classified either way, i.e. $\min P_{best}(\mathbf{x_i^{ny}})-P_{second-best}(\mathbf{x_i^{ny}})$.
  \item \textbf{Highest Loss (HL)} considers the instances which produce the highest values in the loss function $\mathcal{L}$ when compared to their given label meaning they are the hardest to learn, i.e. $\max \mathcal{L}(x_i^{ny}, y_i)$.
\end{enumerate}

%  % \item \textbf{Maximum Entropy (Ent):} It considers the most uncertain instance as the one with the highest conditional entropy with respect to all possible classes, i.e., $\max_{\mathbf{{x_i^{ny}}}} -\sum_{c=1}^C P(y=c|\mathbf{x_i^{ny}}) \log P(y=c|\mathbf{x_i^{ny}})$

\subsection{Active Learner Query Policies}
\label{ssec:policies}
The aforementioned uncertainty measures are used by the active learner in combination with two different policies on how to deplete the query budget over time:

\begin{enumerate}
    \item[] \textbf{Static policy}. The active learner asks a constant number $o(t) = M, \forall t$ of queries at every batch arrival of stream data. Essentially, for each batch, the active learner queries the most uncertain $M$ data instances that are considered noisy by the quality model.

    \item[] \textbf{Dynamic policy}. The active learner dynamically adjusts $o(t)$ based on the value of the loss function of the quality model. The rationale behind is to increase the number of queries when the quality model has a low learning capacity, reflected by high loss function values, and to decrease the number of queries when loss function converges to lower values. Specifically, we propose to adjust $o(t)$ as following:
\begin{equation} \label{eq:1}
    o(t)=o(t-1)(1-\frac{L^{\mathfrak{Q}}(t-2)-L^{\mathfrak{Q}}(t-1)}{L^{\mathfrak{Q}}(t-1)})
\end{equation}
where
%\begin{equation} \label{eq:2}
%    L^{\mathfrak{Q}}(t) = \frac{1}{|\mathbf{\tilde{x}}(t)|}\sum_{x \in \mathbf{\tilde{x}}(t)}\mathcal{L}_e(x, y) 
%\end{equation}
\begin{equation} \label{eq:2}
    L^{\mathfrak{Q}}(t) = \frac{1}{|\mathbf{\tilde{x}}(t)|}\sum_{x_i \in \mathbf{\tilde{x}}}\sum_{c=1}^C p(y=c|\mathbf{x}_i) \log p(y=c|\mathbf{x}_i)
\end{equation}
%\end{equation}
% \begin{equation} \label{eq:2}
%     L^{\mathfrak{Q}_{t-1}}=-\frac{1}{N}\sum_{i=1}^N\sum_{c=1}^C p(y=c|\mathbf{x}_i) \log p(y=c|\mathbf{x}_i)
% \end{equation}
is the average entropy loss across all training samples used at time period $t$. Since the re-training of the model(s) happens after the oracle querying, we use the loss from the time periods $t-1$ and $t-2$. 
Finally, we note that the number of active queries is capped by the given budget $B$, i.e. the number of active queries used is: 
%$L^{\mathfrak{Q}_{t-1}}=-\frac{1}{N}\sum_{i=1}^N\sum_{c=1}^C p(y=c|\mathbf{x}_i) \log p(y=c|\mathbf{x}_i)$ 
\begin{equation}
  \min (B - \sum_{j=1}^{t-1}o(j),o(t))  
\end{equation}
\end{enumerate}

\begin{algorithm}[tb]

\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{Initial dataset $D^I$, Data batches $D$ made of: samples $\mathbf{x}$, given labels $\mathbf{y}$, Budget $B$}

\Output{Quality model $\mathfrak{Q}$, Classifier $\mathfrak{C}$}
\vspace{0.2cm}
Train $\mathfrak{Q}$ and $\mathfrak{C}$ with $D^I$ \\
\vspace{0.2cm}
\ForEach{arriving $D$}{
$y^p$ := Predict label by Quality model $\mathfrak{Q}$ \\ 
$\mathbf{x}^{cl}$ = $\{\forall x_i \in D,  y_i^p = y_i\}$ \\
$\mathbf{x}^{ny}$ = $\{\forall x_i \in D,  y_i^p \neq y_i\}$ \\
\vspace{0.2cm}
$x^{or}$ = Select $o(t)$ samples from $\mathbf{x}^{ny}$ according to Section \ref{ssec:uncertainty} and \ref{ssec:policies} \\
Relabel $x^{os}$ via oracle \\
\vspace{0.2cm}
Train $\mathfrak{Q}$ and $\mathfrak{C}$ with $\mathbf{x}^{cl} \cup \mathbf{x}^{or}$
}

\caption{Quality Driven Active Learning.}
\label{alg:aqlpolicy}
\end{algorithm}

Standard active learning studies query one instance at a time and train the model by adding that instance to the training set. Then the learner queries the next instance based on the retrained model and repeats the procedures recursively until all the budget is spent or the desired performance is achieved. However, in an online setting where data arrives constantly in batches, often it is computationally too expensive to retrain the model after each oracle query and repeat for the next one. Therefore, we decided to query $o(t)$ instances at once and retrain our model just once at each batch arrival. This applies to both policies: static and dynamic. This matches well our online setting where the number of batches is big and models are retrained with new data at each batch arrival.


==> IJCAI-bigtable.tex <==
\begin{table*}[htp]
\caption{Summary of learning accuracy across different datasets, nois ratio: 5 alternative approaches v.s. three different versions of \alg, namely \algns(3), \algns(5), and \algns$^{D}$.  }
\label{tab:bigtable}
\centering
\begin{tabular}{cccccccccc}

\hline
\multicolumn{10}{c}{Initial size = 50}\\
\hline
\multicolumn{1}{c|}{\textbf{Dataset}}   & \multicolumn{1}{c|}{\textbf{Noise}} & \multicolumn{1}{c|}{\textbf{Opt-sel}}    & \multicolumn{1}{c|}{\textbf{No-sel}} & \multicolumn{1}{c|}{\textbf{Q-only}}   & \multicolumn{1}{c|}{\textbf{AL-only(3)}} & \multicolumn{1}{c|}{\textbf{AL-only(5)}} & \multicolumn{1}{c|}{\textbf{\algns(3)}} & \textbf{\algns(5)} & \multicolumn{1}{c}{\textbf{\algns$^{D}$}} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{usps}}       & \multicolumn{1}{c|}{80\%}       & \multicolumn{1}{c|}{87.35}          & \multicolumn{1}{c|}{64.47}  & \multicolumn{1}{c|}{63.79} & \multicolumn{1}{c|}{76.07}      & \multicolumn{1}{c|}{80.60}      & \multicolumn{1}{c|}{82.13} & \multicolumn{1}{c|}{\textbf{87.72}} & \multicolumn{1}{c}{86.1} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{\textbf{90.20}} & \multicolumn{1}{c|}{84.89}  & \multicolumn{1}{c|}{70.32} & \multicolumn{1}{c|}{87.24}      & \multicolumn{1}{c|}{88.39}      & \multicolumn{1}{c|}{86.04} & \multicolumn{1}{c|}{89.62} & \multicolumn{1}{c}{88.54}          \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{pendigits}} & \multicolumn{1}{c|}{80\%}       & \multicolumn{1}{c|}{87.60}          & \multicolumn{1}{c|}{69.88}  & \multicolumn{1}{c|}{71.82} & \multicolumn{1}{c|}{82.31}      & \multicolumn{1}{c|}{86.26}      & \multicolumn{1}{c|}{86.74} & \multicolumn{1}{c|}{\textbf{89.44}} & \multicolumn{1}{c}{87.78} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{90.83}          & \multicolumn{1}{c|}{87.03}  & \multicolumn{1}{c|}{74.98} & \multicolumn{1}{c|}{89.85}      & \multicolumn{1}{c|}{91.35}      & \multicolumn{1}{c|}{88.72} & \multicolumn{1}{c|}{\textbf{91.30}} & \multicolumn{1}{c}{88.8} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{optdigits}} & \multicolumn{1}{c|}{80\%}       & \multicolumn{1}{c|}{95.09}          & \multicolumn{1}{c|}{73.20}  & \multicolumn{1}{c|}{74.72} & \multicolumn{1}{c|}{86.00}      & \multicolumn{1}{c|}{90.40}      & \multicolumn{1}{c|}{93.70} & \multicolumn{1}{c|}{\textbf{96.00}} & \multicolumn{1}{c}{94.78} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{96.57} & \multicolumn{1}{c|}{93.14}  & \multicolumn{1}{c|}{81.45} & \multicolumn{1}{c|}{95.00}      & \multicolumn{1}{c|}{95.76}      & \multicolumn{1}{c|}{96.35} & \multicolumn{1}{c|}{\textbf{96.93}} & \multicolumn{1}{c}{96.36}         \\
\hline
\multicolumn{10}{c}{Initial size = 150}\\
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{letter}} & \multicolumn{1}{c|}{80\%}       & \multicolumn{1}{c|}{\textbf{86.55}}          & \multicolumn{1}{c|}{66.1}  & \multicolumn{1}{c|}{65.25} & \multicolumn{1}{c|}{75.32}      & \multicolumn{1}{c|}{79.26}      & \multicolumn{1}{c|}{83.62} & \multicolumn{1}{c|}{86.35} & \multicolumn{1}{c}{-} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{\textbf{90.25}} & \multicolumn{1}{c|}{82.74}  & \multicolumn{1}{c|}{71.22} & \multicolumn{1}{c|}{85.44}      & \multicolumn{1}{c|}{86.62}      & \multicolumn{1}{c|}{86.27} & \multicolumn{1}{c|}{88.24} & \multicolumn{1}{c}{-}\\

\hline
\multicolumn{10}{c}{Initial size = 150}\\
\hline

\multicolumn{1}{c|}{\multirow{2}{*}{usps}}       & \multicolumn{1}{c|}{80\%}       & \multicolumn{1}{c|}{88.96}          & \multicolumn{1}{c|}{77.49}  & \multicolumn{1}{c|}{86.23} & \multicolumn{1}{c|}{83.52}      & \multicolumn{1}{c|}{85.75}      & \multicolumn{1}{c|}{89.55} & \multicolumn{1}{c|}{\textbf{90.88}} & \multicolumn{1}{c}{89.42} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{90.76} & \multicolumn{1}{c|}{86.84}  & \multicolumn{1}{c|}{88.43} & \multicolumn{1}{c|}{88.75}      & \multicolumn{1}{c|}{91.35}      & \multicolumn{1}{c|}{90.81} & \multicolumn{1}{c|}{\textbf{91.39}} & \multicolumn{1}{c}{90.62}         \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{pendigits}} & \multicolumn{1}{c|}{80\%}       & \multicolumn{1}{c|}{89.30}          & \multicolumn{1}{c|}{81.74}  & \multicolumn{1}{c|}{86.04} & \multicolumn{1}{c|}{82.31}      & \multicolumn{1}{c|}{89.92}      & \multicolumn{1}{c|}{90.94} & \multicolumn{1}{c|}{\textbf{92.02}} & \multicolumn{1}{c}{90.63} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{90.83}          & \multicolumn{1}{c|}{91.68}  & \multicolumn{1}{c|}{89.42} & \multicolumn{1}{c|}{87.48}      & \multicolumn{1}{c|}{91.16}      & \multicolumn{1}{c|}{91.69} & \multicolumn{1}{c|}{\textbf{92.90}} & \multicolumn{1}{c}{92.2} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{optdigits}} & \multicolumn{1}{c|}{80\%}       & \multicolumn{1}{c|}{95.91}          & \multicolumn{1}{c|}{87.43}  & \multicolumn{1}{c|}{94.91} & \multicolumn{1}{c|}{92.27}      & \multicolumn{1}{c|}{94.15}      & \multicolumn{1}{c|}{96.77} & \multicolumn{1}{c|}{\textbf{97.26}} & \multicolumn{1}{c}{96.37} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{96.88} & \multicolumn{1}{c|}{94.39}  & \multicolumn{1}{c|}{95.99} & \multicolumn{1}{c|}{95.92}      & \multicolumn{1}{c|}{96.46}      & \multicolumn{1}{c|}{97.17} & \multicolumn{1}{c|}{\textbf{97.49}}  & \multicolumn{1}{c}{96.5}         \\ 
\hline
\multicolumn{10}{c}{Initial size = 450}\\
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{letter}} & \multicolumn{1}{c|}{80\%}       & \multicolumn{1}{c|}{87.28}          & \multicolumn{1}{c|}{70.43}  & \multicolumn{1}{c|}{79.12} & \multicolumn{1}{c|}{77.66}      & \multicolumn{1}{c|}{80.74}      & \multicolumn{1}{c|}{86.27} & \multicolumn{1}{c|}{\textbf{88.4}} & \multicolumn{1}{c}{-} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{\textbf{90.61}} & \multicolumn{1}{c|}{84.08}  & \multicolumn{1}{c|}{82.18} & \multicolumn{1}{c|}{87.18}      & \multicolumn{1}{c|}{88.4}      & \multicolumn{1}{c|}{86.27} & \multicolumn{1}{c|}{89.57}  & \multicolumn{1}{c}{-}\\
\hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> IJCAI-bigtable_cifar.tex <==
\begin{table*}[tp]
\caption{Summary of learning accuracy across different datasets and noise ratios. Five alternative approaches v.s. two different static versions of \alg, namely \algns(5\%) and \algns(10\%) using BvSB.}
\label{tab:bigtable_cifar}
\centering
\centering
\begin{tabular}{ccccccccc}

\hline
\multicolumn{1}{c|}{{Dataset}} &
\multicolumn{1}{c|}{\textbf{Noise}} & \multicolumn{1}{c|}{\textbf{Opt-sel}}    & \multicolumn{1}{c|}{\textbf{No-sel}} & \multicolumn{1}{c|}{\textbf{Q-only}}   & \multicolumn{1}{c|}{\textbf{AL-only($5\%$)}} & \multicolumn{1}{c|}{\textbf{AL-only($10\%$)}} & \multicolumn{1}{c|}{\textbf{\algns($5\%$)}} & \textbf{\algns($10\%$)} \\ \hline \hline

\multicolumn{1}{c|}{\multirow{2}{*}{CIFAR-10}} &
\multicolumn{1}{c|}{30\%}  & \multicolumn{1}{c|}{78.25} & \multicolumn{1}{c|}{54.92}  & \multicolumn{1}{c|}{65.32} & \multicolumn{1}{c|}{55.56}      & \multicolumn{1}{c|}{57.33}      & \multicolumn{1}{c|}{75.98} & \multicolumn{1}{c}{74.00} \\
\multicolumn{1}{c|}{} &
\multicolumn{1}{c|}{60\%}  & \multicolumn{1}{c|}{78.32}          & \multicolumn{1}{c|}{55.2}  & \multicolumn{1}{c|}{64.62} & \multicolumn{1}{c|}{56.04}      & \multicolumn{1}{c|}{56.11}      & \multicolumn{1}{c|}{70.71} & \multicolumn{1}{c}{74.07} \\ \hline

\multicolumn{1}{c|}{\multirow{2}{*}{CIFAR-100}} &
\multicolumn{1}{c|}{30\%}       & \multicolumn{1}{c|}{39.28}          & \multicolumn{1}{c|}{32.12}  & \multicolumn{1}{c|}{4.41} & \multicolumn{1}{c|}{32.10}      & \multicolumn{1}{c|}{32.14}      & \multicolumn{1}{c|}{39.10} & \multicolumn{1}{c}{36.55} \\
\multicolumn{1}{c|}{}  &
\multicolumn{1}{c|}{60\%}       & \multicolumn{1}{c|}{37.64} & \multicolumn{1}{c|}{14.48}  & \multicolumn{1}{c|}{4.15} & \multicolumn{1}{c|}{33.98}      & \multicolumn{1}{c|}{34.92}      & \multicolumn{1}{c|}{37.04} & \multicolumn{1}{c}{38.40} \\ \hline

\end{tabular}
\end{table*}




==> IJCAI-cifar_dynamic_table.tex <==
\begin{table}
\caption{Comparison of static and dynamic versions of \alg with 5\% query budget per batch of arriving data stream. \rb{double check if results correct}}
\label{tab:cifar_dynamictab}
\centering
% \resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{cccc}
\hline
\multicolumn{1}{c|}{\textbf{Dataset}} &
\multicolumn{1}{c|}{\textbf{Noise}} &  \multicolumn{1}{c|}{\textbf{\algns($5\%$)}} & \multicolumn{1}{c}{\textbf{\algns$^{D}$}} \\ \hline \hline

\multicolumn{1}{c|}{\multirow{2}{*}{CIFAR-10}} &
\multicolumn{1}{c|}{30\%} &
\multicolumn{1}{c|}{75.98} & \multicolumn{1}{c}{72.45}          \\ 

\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{60\%} & 
\multicolumn{1}{c|}{70.71} & \multicolumn{1}{c}{71.82} \\ \hline

% \multicolumn{1}{c|}{\multirow{2}{*}{CIFAR-100}} &
% \multicolumn{1}{c|}{30\%} &
% \multicolumn{1}{c|}{-} & \multicolumn{1}{c}{-}          \\ 

% \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{60\%} & 
% \multicolumn{1}{c|}{-} & \multicolumn{1}{c}{-} \\ \hline

\end{tabular}
% }
\end{table}

==> IJCAI-dynamic_table.tex <==
\begin{table}
\caption{Results of SVM classifier: summary of learning accuracy across different datasets, noise ratios. Comparison of static and dynamic versions of \alg with 3 query budget per epoch, namely  namely \algns(3) and \algns$^{D}$.  }
\label{tab:dynamictab}
\centering
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{cccc}
\hline
\multicolumn{4}{c}{Initial size = 50}\\
\hline
\multicolumn{1}{c|}{\textbf{Dataset}}   & \multicolumn{1}{c|}{\textbf{Noise}} &  \multicolumn{1}{c|}{\textbf{\algns(3)}} & \multicolumn{1}{c}{\textbf{\algns$^{D}$}} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{usps}}       & \multicolumn{1}{c|}{80\%} & \multicolumn{1}{c|}{82.13} & \multicolumn{1}{c}{86.10} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%} & \multicolumn{1}{c|}{86.04} & \multicolumn{1}{c}{88.54}          \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{pendigits}} & \multicolumn{1}{c|}{80\%} & \multicolumn{1}{c|}{86.74} &  \multicolumn{1}{c}{87.78} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%} & \multicolumn{1}{c|}{88.72} & \multicolumn{1}{c}{88.8} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{optdigits}} & \multicolumn{1}{c|}{80\%} & \multicolumn{1}{c|}{93.70}  & \multicolumn{1}{c}{94.78} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%} & \multicolumn{1}{c|}{96.35} & \multicolumn{1}{c}{96.36}         \\
\hline
\multicolumn{4}{c}{Initial size = 150}\\
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{usps}}       & \multicolumn{1}{c|}{80\%}    & \multicolumn{1}{c|}{89.55} & \multicolumn{1}{c}{89.42} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}    & \multicolumn{1}{c|}{90.81} & \multicolumn{1}{c}{90.62}         \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{pendigits}} & \multicolumn{1}{c|}{80\%} & \multicolumn{1}{c|}{90.94} & \multicolumn{1}{c}{90.63} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%}    & \multicolumn{1}{c|}{91.69} & \multicolumn{1}{c}{92.2} \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{optdigits}} & \multicolumn{1}{c|}{80\%} & \multicolumn{1}{c|}{96.77}  & \multicolumn{1}{c}{96.37} \\
\multicolumn{1}{c|}{}                            & \multicolumn{1}{c|}{60\%} & \multicolumn{1}{c|}{97.17}  & \multicolumn{1}{c}{96.5}         \\ 
\hline
\end{tabular}
}
\end{table}
